Diversity Measures: Domain-Independent Proxies for Failure in Language Model Queries

Error prediction in large language models often relies on domain-specific information. In this paper, we present measures for quantification of error in the response of a large language model based on the diversity of responses to a given prompt - hence independent of the underlying application. We describe how three such measures - based on entropy, Gini impurity, and centroid distance - can be employed. We perform a suite of experiments on multiple datasets and temperature settings to demonstrate that these measures strongly correlate with the probability of failure. Additionally, we present empirical results demonstrating how these measures can be applied to few-shot prompting, chain-of-thought reasoning, and error detection.

==> old_stuff.tex <==
%\subsection{Enhanced Self-consistency}
%Here we look to replace the selection criteria for self-consistency (Equation~\ref{eqn:majVote}) with an alternative.  We examine for set-based and vector-based output as follows.
%\vspace{10pt}

%\noindent\textbf{Set-Based Output.}  

%\begin{eqnarray}
%\arg \min_i - \sum_{e \in \ba_i}P(e)\log(P(e))\\
%\arg \min_i 1-\sum_{e \in \ba_i}P(e)^2
%\end{eqnarray}

%Alternatively, we can pick the response from the model that is closest to the intersection of the result.
%\begin{eqnarray}
%\arg \min_i \frac{|\ba_i|}{|\cap_j \ba_j|}
%\end{eqnarray}

%\noindent\textbf{Vector-Based Output.}  In this case, Equation~\ref{eqn:majVote} by the selection of the response closest to the centroid.
%\begin{eqnarray}
%\arg \min_i d(\embed(a_i),\cent)
%\end{eqnarray}

